Weight of Evidence as a Basis for Human-Oriented Explanations

Interpretability is an elusive but highly sought-after characteristic of modern machine learning methods. Recent work has focused on interpretability via $\textit{explanations}$, which justify individual model predictions. In this work, we take a step towards reconciling machine explanations with those that humans produce and prefer by taking inspiration from the study of explanation in philosophy, cognitive science, and the social sciences. We identify key aspects in which these human explanations differ from current machine explanations, distill them into a list of desiderata, and formalize them into a framework via the notion of $\textit{weight of evidence}$ from information theory. Finally, we instantiate this framework in two simple applications and show it produces intuitive and comprehensible explanations.

==> approach.tex <==
\section{A general framework for correspondence across hyperbolic spaces}
\label{sec:approach}

%\subsection{Matching with complex learnable registration functions}
The failure of the baseline Euclidean alignment methods (and their hyperbolic versions) discussed in the previous section, combined with the underlying branch permutability invariance responsible for it, make it clear that the space of registration transformations $\cF$ in Problem~\eqref{eq:invariant_wasserstein} has to be generalized not only beyond orthogonality but beyond linearity too. Ideally we would want to search for $f$ among all continuous mappings between $\cY$ and $\cX$, i.e, letting $\cF=\{f:\cY \rightarrow \cX \suchthat f\in \mathcal{C}(\cY)\}$. To make this search computationally tractable, we can instead approximate this function class with deep neural networks $f_\theta$ parametrized by $\theta \in \Theta$. 
While an alternating minimization approach is still possible, solving a minimization for $\theta$ to completion in each iteration is undesirable. Instead, we can reverse the order of optimization and rewrite our objective as
\begin{equation}\label{eq:invariant_wasserstein_two}
    \min_{f_{\theta} \in \cF} \min_{\pi \in \Pi(\alpha, \beta)} \int_{\cX \times \cX} d(x,f(y)) d\pi(x,f(y)) = \min_{f_{\theta} \in \cF}  \text{W}_{\epsilon}(\alpha, f_{\theta}^{\#}\beta).
\end{equation}
Since  $\text{W}(\alpha, f_{\theta}^{\#}\beta)$ is differentiable with respect to $\theta$, we can use gradient-descent based methods to optimize it. Wasserstein distances have been used before as loss functions, particularly in the context of deep generative modeling \citep{Arjovsky2017Wasserstein, genevay2018learning,salimans2018improving}. When used as a loss function, the entropy-regularized version (Eq.~\eqref{eq:entreg_wasserstein}) has the undesirable property that $\text{W}_{\epsilon}(\alpha, \alpha) \neq 0$, in addition to having biased sample gradients \citep{bellemare2017cramer}. Following \citet{genevay2018learning}, we instead consider the \textit{Sinkhorn Divergence}:
\begin{equation}\label{eq:sinkhorn_divergence}
    \text{SD}_{\epsilon}(\alpha, \beta) \triangleq \text{W}_{\epsilon}(\alpha,\beta) - \frac{1}{2}\bigl( \text{W}_\epsilon(\alpha, \alpha) + \text{W}_{\epsilon}(\beta,\beta) \bigr).
\end{equation}
Besides being a proper divergence and providing unbiased gradients, this function is convex, smooth and positive-definite \citep{feydy2019interpolating}, and its sample complexity is well characterized \citep{genevay2019sample}, all of which make it an appealing loss function. Thus, we can replace it in Problem \eqref{eq:invariant_wasserstein_two}, yielding our final objective:
\begin{equation}\label{eq:objective}
    \min_{\theta: f_{\theta}[\mathbb{D}^d] \subseteq \mathbb{D}^d} \text{SD}_{\epsilon}(\alpha, f_{\theta}^{\#}\beta). %=  \min_{\theta: f_{\theta}[\cM] \subseteq \cM }  \int_{\cX \times \cX} d_{\cX}(x,f_{\theta}(y)) d\pi(x,f_{\theta}(y)) + \epsilon 
\end{equation}

The last remaining challenge is that we need to construct a class of neural networks that parametrizes $\cF := \{f_\theta \suchthat f_\theta(\mathbb{D}^d) \subseteq \mathbb{D}^d\}$, i.e., functions that map $\mathbb{D}^d$ onto itself. In recent work, \citet{ganea2018hyperbolic} propose a class of hyperbolic neural networks that do exactly this. As they point out, the basic operations in hyperbolic space that we introduced in \secref{sec:background} suffice to define analogues of various differentiable building blocks of traditional neural networks. For example, a hyperbolic linear layer can be defined as $f_{\textsc{HyperLin}}(\x; \W, \mathbf{b})\triangleq  (\W\otimes \x) \oplus \mathbf{b} = \exp_0(\W\log_0(\x)) \oplus \mathbf{b}$. Analogously, a layer applying a nonlinearity $\sigma(\cdot)$ in the hyperbolic sense can be defined as $\sigma_{\mathbf{D}}(\x) \triangleq \exp_0(\sigma\log_0(\x))$. Here, we also consider \textit{M\"obius Transformation layers}, $f_{\text{M\"obius}}(\x) = \P(\v \oplus \x)$, with $\P \in \text{SO}(d)$ and $\v \in \mathbb{D}^d$. With these building blocks, we can parametrize highly nonlinear functions $f_{\theta}: \mathbb{D}^n \rightarrow \mathbb{D}^n$ as a sequence of such hyperbolic layers, e.g., $\mathbf{h}^{(i)} = \sigma_{\mathbb{D}} ( \W^{(i)}\otimes \mathbf{h}^{(i-1)} \oplus \mathbf{b}^{(i)})$. Note that for the hyperbolic linear layer---but crucially, not for the M\"obius layer---the intermediate hidden states $\mathbf{h}^{(i)}$ need not live in the same dimensional space as the input and output, i.e., using rectangular weight matrices $\W$ we can map intermediate states to Poincar\'e balls of different dimensionality.

\paragraph{Optimization}
Evaluation of the loss function in \eqref{eq:objective} is itself an optimization problem, i.e., solving instances of regularized optimal transport. We backpropagate through this objective as proposed by \citet{genevay2018learning}, using the \texttt{geomloss} toolbox for efficiency. For the outer-level optimization, we rely on Riemannian gradient descent \citep{zhang2016riemannian, wilson2018gradient}. We found that the adaptive methods of \citet{becigneul2019riemannian} worked best, particularly \textsc{Radam}. Note that for the \textsc{HyperLinear} layers only the bias term is constrained (on the Poincar\' Ball), while for our \textsc{M\"obius} layers the weight matrix is also constrained (in the Stiefel manifold), so for the latter we optimize over the product of these two manifolds. Additional details on optimization are provided in the Appendix.

\paragraph{Avoiding poor local minima}
The loss function \eqref{eq:objective} is highly non-convex with respect to $\theta$, a consequence of both the objective itself and the nature of hyperbolic neural networks \citep{ganea2018hyperbolic}. As a result, we found that initialization plays a crucial role in this problem, since it is very hard to overcome a poor initial local minimum. Even suitable layer-wise random initialization of weights and biases proved futile. As a solution, we experimented with three pre-training initialization schemes, that roughly ensure (in different ways) that $f$ does not initially ``collapse'' the space $\cY$ (details provided in Appendix~\ref{sec:pretrain}). In addition, following \citep{alvarez-melis2019invariances}, we use an annealing scheme on the entropy-regularization parameter $\epsilon$. Starting from an aggressive regularization (large $\epsilon_0$), we gradually decrease it with a fixed decay rate $\epsilon_t = \xi \cdot \epsilon_{t-1}$. In all our experiments we use $\xi = 0.99$.



==> background.tex <==
\section{Weight of Evidence}
\label{sec:background}

In the previous section, we proposed desideratta for an interpretability framework. We show that the Weight of Evidence is a simple and well-understood concept which shares these desideratta, making it an ideal tool to formalize this framework.


The \textbf{Weight of Evidence} (WoE) is an information theoretic approach to analyze variable effects in prediction models. It traces its origin to Turing and Shannon (or even before that), has been re-discovered in many contexts, but the name most associated with it is I.J. Good, who claims ideas like it go back to at least Pierce (1878). 

Good it as follows. For a hypothesis $h$ and evidence $e$, the weight-of-evidence (woe) is given by
\begin{equation}\label{eq:woe_def}
    \text{woe}(h : e) \triangleq  \log \frac{O( h \mid e) }{O(h)}
\end{equation}
where $O(\cdot)$ are the log-odds, i.e.,
\begin{equation}
    O(h) := \frac{p(h)}{p(\bar{h})}, \qquad O( h \mid e) := \frac{p(h \mid e)}{p(\bar{h} \mid e)}
\end{equation}
The interpretation of \eqref{eq:woe_def} is simple. If $\text{woe}(h:e) > 0 $ then $h$ is more likely under $e$ than marginally, i.e., the evidence \textit{speaks in favor of hypothesis} $h$. Analogously, $\text{woe}(h:e) < 0 $ indicates $h$ is less likely when taking into account the evidence than it was without it.

The WoE can be conditioned 
\begin{equation}
    \text{woe}(h : e \mid c) \triangleq  \log \frac{O( h \mid e, c) }{O(h \mid c)}
\end{equation}
and can be computed relative to an arbitrary alternative hypothesis (i.e., not necessarily the complement):
\begin{equation}
        \text{woe}(h/h': e) \triangleq  \text{woe}(h: e \mid h \lor h')
\end{equation}
Thus, more generally, we can interpret $\text{woe}$ as the "evidence in favor of $h$ against $h'$ provided by $e$ (and perhaps conditioned on $c$).

\subsection{Axiomatic Derivation}

Good proposes the following desiderata on Weight of Evidence:
\begin{enumerate}
    \item WoE should be function of the likelihoods, i.e., $$\text{woe} = f[p(e\mid h), p(e\mid \bar{h})]$$
    \item The posterior should be a function of prior and WoE: $$p(h\mid e) = g [p(h), \text{woe}(h : e)]$$
    \item WoE should be additive (on the evidence): $$\text{woe}(h : e_1 \land e_2) = \text{woe}(h :e_1) + \text{woe} (h: e_2 \mid e_1)$$
\end{enumerate}
He then shows that the only (up to a constant factor) function of $e$ and $h$ that satisfies (1)-(3) is \eqref{eq:woe_def}. 

\subsection{Connection to Bayes' Rule}
Assume for simplicity that $h: Y=1$, $\bar{h}: Y = 0$ and $e= X$. Simple algebraic manipulation of \eqref{eq:woe_def} yields:
\begin{equation}
    \log \frac{P(Y=1 \mid X)}{P(Y=0 \mid X)} = \underbrace{\log\frac{P(Y=1)}{P(Y=0)}}_{\text{Sample log-odds}} + \underbrace{\log \frac{P(X \mid Y=1)}{P(X \mid Y=0)}}_{\textit{Weight of evidence}}
\end{equation}
The interpretation of the expression above is clear: the greater the WOE, the higher the chance of observing $Y=1$. The log makes the interpretation particularly simple:
\begin{itemize}
    \item WOE $> 0 \then P(Y=1)$ is \textbf{above} average (w.r.t to the sample odds) 
    \item WOE $< 0 \then P(Y=1)$ is \textbf{below} average (w.r.t to the sample odds)
\end{itemize}
It can be directly extended to the multi-variate setting using a the Naive Bayes (conditional independence assumption) yielding:
\begin{equation}
    \log \frac{P(Y=1 \mid X)}{P(Y=0 \mid X)} = \log\frac{P(Y=1)}{P(Y=0)} + \sum_{i=1}^n \log \frac{P(X_i \mid Y=1)}{P(X_i \mid Y=0)}
\end{equation}
Its connection to Naive-Bayes classifiers is immediate. The NB models says that:
\begin{equation*}
    \text{conditional log-odds} = \text{sample log-odds} + \text{sum of per-variable WOE values}
\end{equation*}
Thus, WOE can be understood as evidence for/against $H_1: Y=1$ provided by each variable.



WOE can be leveraged to measure overall predictive strength of each variable by means of the \textbf{Information Value}:
\begin{equation*}
    \underbrace{\text{Information Value}(X_i)}_{\approx \text{weighted sum of WOE's}} \triangleq \int_{X_i} \log \frac{P(X_i \mid Y=1)}{P(X_i \mid Y=0)} \bigl[ P(X_i \mid Y=0) - P(X_i \mid Y=0) \bigr] dx
\end{equation*}
Thus, IV can be understood as a measure of how well variable $X_i$ helps us separate $Y=1$ from $Y=0$. In applied settings, a commonly-used rule of thumb says that if $IV < 0.05$ then the variable has little predictive power. \textbf{Note:} This is a \textit{global} property, and thus probably not of interest in our setting (+ intractable in most cases). Including it here for completion.

\subsection{Computing WOE}

Some useful properties:
\begin{enumerate}
    \item $\woe(h/h' : e) = \log \frac{P(e \mid h)}{P(e\mid h')}$
    \item $\argmax_e \woe(h/h' : e) = \argmax_e \log \frac{P(e\mid h)}{P(e \mid h')} = \argmax \log \frac{P(h\mid e}{P(h'\mid e)}$
    \item $\woe(h/h' : e_2 \mid e_1) = \log \frac{P(e_2 \mid h, e_1)}{P(e_2 \mid h', e_1)}$
    \item $\woe(h/h': e_1 \land e_2) = \log \frac{P(e_1 \mid h)}{P(e_1\mid h')} + \log \frac{P(e_2 \mid h, e_1)}{P(e_2 \mid h', e_1)}$
    \item $\woe(h/h': e_1 \land e_2 \land \dots \land e_n) = \sum_{i=1}^n \log \frac{P(e_i \mid e_{i-1}, \dots, e_1, h)}{P(e_i \mid e_{i-1}, \dots, e_1, h')}$
\end{enumerate}

\begin{obs}
    Note that we have two ways to compute $\woe$ for multi-variate (composite) evidence. The identity in (5) and directly on the "total" evidence $\vec{e}$: $\woe(h/h': \vec{e}) = \log \frac{P(\vec{e} \mid h)}{P(\vec{e} \mid h')}$
\end{obs}


==> estimation.tex <==
\section{Estimating Weight of Evidence Scores for Black-Box Models}


\iffalse
To compute WOE we need to be able to compute either $P(e|h)$ or $P(h \mid e)$ for any $e$ and $h$. In our case, $e$ will be attributes $\vec{x}_{S}$. For hypothesis classes of the type defined above, our goal is thus to estimate $P( \vec{x}_{S}  \mid y)$ [TODO: justify why not the opposite]. This is a (conditional) density estimation problem, but with the unique characteristic that we seek not the density of a single block of variables, 
\fi

For any pair of entailed and contrast hypothesis class, equation \eqref{eq:} provides an exact method to compute the conditional weight of evidence. In order to use this expression, we need to be able to compute $P(X_{S_i} \mid X_{S_{i-1}}, \dots, X_{S_1}, Y \in C)$ for any order of attributes $\{X_{S_i}\}_{i=1}^n$ and outcome set $C$. In an ideal scenario, the prediction model itself would compute and store these values (e.g., in an auto-regressive generative model). In that case, there isn't much left to discuss.

Unfortunately, most prediction models do not compute such probabilities explicitly, so any realistic application of the WoE methodology to interpretability must provide a fallback method to estimate these, independently, from data. Here, we do so for the most challenging setting of a black-box prediction model, assuming access only to additional training data and oracle access to the prediction model.

Our proposed approach relies on training, as a preliminary step, an autoregressive conditional likelihood estimation model (henceforth referred to simply as the \textit{likelihood model}). The training data for this model consists of pairs ($X, \hat{y}$), where $X$ is a sample from the input distribution $X \sim P_X$ and $\hat{y} = f(X)$ is a class label prediction obtained with the prediction model. 


